Memory-Assisted Quantized LDPC Decoding

We enhance coarsely quantized LDPC decoding by reusing computed check node messages from previous iterations. Typically, variable and check nodes update and replace old messages every iteration. We show that, under coarse quantization, discarding old messages entails a significant loss of mutual information. The loss is avoided with additional memory, improving performance by up to 0.23 dB. We optimize quantization with a modified information bottleneck algorithm that considers the statistics of old messages. A simple merge operation reduces memory requirements. Depending on channel conditions and code rate, memory assistance enables up to 32 % better area efficiency for 2-bit decoding.

==> showframetwocolumn.tex <==
\usepackage{showframe}
\usepackage{etoolbox}

\newlength\Fcolumnseprule
\setlength\Fcolumnseprule{0.4pt}

\makeatletter
\newcommand\ShowInterColumnFrame{
	\patchcmd{\@outputdblcol}
	{{\normalcolor\vrule \@width\columnseprule}}
	{\vrule \@width\Fcolumnseprule\hfil
		{\normalcolor\vrule \@width\columnseprule}
		\hfil\vrule \@width\Fcolumnseprule
	}
	{}
	{}
}

\makeatother
\ShowInterColumnFrame

